Charge collection properties of prototype sensors for the LHCb VELO upgrade

An extensive sensor testing campaign is presented, dedicated to measuring the charge collection properties of prototype candidates for the Vertex Locator (VELO) detector for the upgraded LHCb experiment. The charge collection is measured with sensors exposed to fluences of up to $8 \times 10^{15}~1~\mathrm{\,Me\kern -0.1em V}~ \mathrm{ \,n_{eq}}~{\mathrm{ \,cm}}^{-2}$, as well as with nonirradiated prototypes. The results are discussed, including the influence of different levels of irradiation and bias voltage on the charge collection properties. Charge multiplication is observed on some sensors that were nonuniformly irradiated with 24 GeV protons, to the highest fluence levels. An analysis of the charge collection near the guard ring region is also presented, revealing significant differences between the sensor prototypes. All tested sensor variants succeed in collecting the minimum required charge of 6000 electrons after the exposure to the maximum fluence.

==> 00_preamble.tex <==
% THis file contains all the default packages and modifications for
% LHCb formatting

%% %%%%%%%%%%%%%%%%%%
%%  Page formatting
%% %%%%%%%%%%%%%%%%%%
\textheight=230mm
\textwidth=160mm
\oddsidemargin=7mm
\evensidemargin=-10mm
\topmargin=-10mm
\headsep=20mm
\columnsep=5mm
\addtolength{\belowcaptionskip}{0.5em}

\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.99}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}


\setlength{\hoffset}{-2cm}
\setlength{\voffset}{-2cm}
% Page defaults ...
\topmargin=0.5cm
\oddsidemargin=2.5cm
\textwidth=16cm
\textheight=22cm
% Allow the page size to vary a bit ...
\raggedbottom
% To avoid Latex to be too fussy with line breaking ...
\sloppy

%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%% 
\usepackage{microtype}
\usepackage{lineno}  % for line numbering during review
\usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbold
\usepackage{caption} %these three command get the figure and table captions automatically small
\renewcommand{\captionfont}{\small}
\renewcommand{\captionlabelfont}{\small}

%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
\usepackage{color}
\usepackage{colortbl}
\graphicspath{{./figs/}} % Make Latex search fig subdir for figures

%% Math
\usepackage{amsmath} % Adds a large collection of math symbols
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/viewtopic.php?f=5&t=163
%%
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
\expandafter\let\csname oldend#1\expandafter\endcsname\csname
end#1\endcsname
 \renewenvironment{#1}%
   {\linenomath\csname old#1\endcsname}%
   {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
\patchBothAmsMathEnvironmentsForLineno{eqnarray}%
}

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.
\usepackage{hyperref}    % Hyperlinks in references
\usepackage[all]{hypcap} % Internal hyperlinks to floats.


% Make this the last packages you include before the \begin{document}
\usepackage{cite} % Allows for ranges in citations
\usepackage{mciteplus}
\usepackage{subfig}


==> mciteplus/README <==


September 13, 2013

The mciteplus LaTeX package is an enhanced reimplementation of
Thorsten Ohl's mcite package:

http://www.ctan.org/tex-archive/macros/latex/contrib/mcite/

which provides support for the grouping of multiple citations together
as is often done in physics journals. An extensive set of features
provide for other applications such as reference sublisting.

Mciteplus offers the following features, many of which are not available
with the original mcite:

 1. Entry punctuation can be controlled by the bibstyle (.bst) as well
    as the user.

 2. No "double periods" when an entry already ends with a period
    (e.g., an abbreviated journal name).

 3. Support for sublists.

 4. Support for multiple bibliographies and/or auxiliary files.

 5. The bibliography sample label width is automatically updated to
    account for the changes in the numbering due to the grouped entries.
    Maximum label width information is available to user.

 6. Compatible with the natbib package. (The bibstyle must support both
    mciteplus as well as natbib.)

 7. Compatible with the REVTeX4 class. (The bibstyle must support both
    mciteplus as well as natbib.)

 8. Support for the optional argument of \cite[]{}.

 9. Provides a means to allow users to use almost any cite command via
    custom command wrappers and the ability to manually disable all
    automatic internal hooks.

10. Mciteplus compatible sorting bibstyles are possible via the use of a
    "mcitetail" field in the BibTeX database entries.


Please note that existing mcite bibstyles (.bst files) are not compatible
with mciteplus. They will have to be remodified as explained in the
mciteplus documentation.

See the mciteplus_doc.pdf user manual for full details.

For helpful tips, answers to frequently asked questions and other support,
visit the Mciteplus home page at my website:

http://www.michaelshell.org/tex/mciteplus/


Enjoy!

Michael Shell


*******
Version 1.2 (2013/09/13) changes:

 1) Add support for \citenum of natbib version 8.0 and later.
    Thanks to Joseph Wright for reporting this.

 2) Corrected bug with cross-referenced entries with backref.sty.
    Thanks to Martin Böttcher for reporting this problem.

********************************** Files **********************************

README              - This file.

changelog.txt       - Version history.

mciteplus.sty       - The mciteplus LaTeX package.

mciteplus_doc.pdf   - The mciteplus user manual.

mciteplus_doc.tex   - LaTeX source code for the user manual.

mciteplus_code.txt  - Selected .bst modification and other code listings.

apsrevM.bst         - An mciteplus compatible version of REVTeX4's 
                      apsrev.bst.

apsrmpM.bst         - An mciteplus compatible version of REVTeX4's 
                      apsrmp.bst. Note: This is a sorting style. For it to
                      work properly, you must set the "mcitetail" BibTeX
                      database field for every tail entry.

IEEEtranM.bst       - An mciteplus compatible version of IEEEtran.bst.

IEEEtranMN.bst      - An mciteplus compatible version of IEEEtranN.bst
                      (natbib compatible).

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE!
User assumes all risk.
In no event shall any contributor to this code be liable for any damages or
losses, including, but not limited to, incidental, consequential, or any
other damages, resulting from the use or misuse of any information contained
here.

All comments are the opinions of their respective authors.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: mciteplus.sty, mciteplus_doc.pdf, mciteplus_doc.tex,
                   mciteplus_code.txt, apsrevM.bst, apsrmpM.bst,
                   IEEEtranM.bst, IEEEtranMN.bst

***************************************************************************

